Multiple Instance Learning for Detecting Anomalies over Sequential Real-World Datasets

Detecting anomalies over real-world datasets remains a challenging task. Data annotation is an intensive human labor problem, particularly in sequential datasets, where the start and end time of anomalies are not known. As a result, data collected from sequential real-world processes can be largely unlabeled or contain inaccurate labels. These characteristics challenge the application of anomaly detection techniques based on supervised learning. In contrast, Multiple Instance Learning (MIL) has been shown effective on problems with incomplete knowledge of labels in the training dataset, mainly due to the notion of bags. While largely under-leveraged for anomaly detection, MIL provides an appealing formulation for anomaly detection over real-world datasets, and it is the primary contribution of this paper. In this paper, we propose an MIL-based formulation and various algorithmic instantiations of this framework based on different design decisions for key components of the framework. We evaluate the resulting algorithms over four datasets that capture different physical processes along different modalities. The experimental evaluation draws out several observations. The MIL-based formulation performs no worse than single instance learning on easy to moderate datasets and outperforms single-instance learning on more challenging datasets. Altogether, the results show that the framework generalizes well over diverse datasets resulting from different real-world application domains.

==> Sections/oldResults.tex <==
\section{Results}
\label{sec:Results}
\subsection{Datasets}
To show the generalizability of the framework, extensive experiments are conducted on five datasets from various domains. This section summarizes the datasets. 

\subsubsection{Case Western Reserve University (CWRU)}
The CWRU Bearing Database serves as a standardized dataset for pattern classification with mechanical systems. This dataset has known ground-truth labels associated with inherent mechanical states and consists of continuous motor-bearing responses. Five motor-bearing condition states are used which include a normal baseline and four damaged bearing inner fault conditions (IR:0.007, IR:0.014, IR:0.021 and IR:0.028). More detail about this dataset can be found in~\cite{yang2018bearing}.
Motor-load variations were not considered in the study based on their relatively low impact to bearing excitation~\cite{SMITH2015100}. All four damaged states measurements are considered as anomalies in our settings.  

We consider data with 1797 Rotations Per Minute (rpm) sampled at 12k Hz meaning almost 30 rotations per second. Signals are segmented by $400$ window size which creates an instance from one motor revolution. This leads to 1853 data points. 300 points from normal state are utilized for training set, while the rest served as test set. In order to achieve an almost balanced number of normal and anomalous test bags, 10 rotations are included in normal bags (30 bags) while 35 rotations (almost 1 second of measurements) are considered for damaged/anomalous ones (30 normal vs. 35 anomalous bags). 

Since CWRU is known as a clean dataset and it is important to evaluate the robustness of the proposed algorithm to noise, we corrupt the ground-truth by various levels of Gaussian white noise (20, 10, 5, and 1 Signal to Noise Ratio (SNR)). This allows us to employ the CWRU dataset as control to evaluate the proposed methodology on a well-understood and characterized dataset.

\subsubsection{Smartphone-Based Recognition of Human Activities and Postural Transitions Data Set (HAPT)}
HAPT is a public labelled dataset obtained from basic activities performed by 30 volunteers. Activities include static (sitting, standing, lying), dynamic (walking, walking downstairs and upstairs), and postural transitions between the static postures (sit to lie, lie to sit, stand to sit, sit to stand, stand to lie, lie to stand).   
The sensor measurements are captured by a smartphone and pre-processed by applying filters and using fixed-length sliding window with overlap.
Each data point is a 561-featured vector containing time and frequency domain variables. Interested readers can find more details from this experiment in~\cite{reyes2016transition}. The dataset is available in UCI repository~\cite{Dua:2019}.  

In this setting, we define postural transition instances as anomalous activities, but it is noticeable that can be substituted by any other ones. According to this definition, out of 10929 data points, 518 instances are anomalous. 
To form the training and test bags with balanced number of normal points and anomalies, 104 training bags are extracted from 5200 normal instances (static and dynamic activities,) while 104 test bags are formed from remaining 5211 data points for test set. Length of the bags are 50.
Then, 518 outliers are randomly inserted to half of the test bags and generate 52 normal and anomalous bags. 

\subsubsection{Virat Video Dataset}
Virat is a well-known public dataset appropriate for real-world video surveillance. It contains data collected from multiple outdoor scenes showing people doing normal activities. A stationary camera is placed in a scene while a variety of movers and background activities are captured over time. The main purpose of the dataset is to recognize activities. Details of the dataset are given in~\cite{oh2011large}. 

One out of 16 scenes exist in the Virat is considered in our experiment. There are multiple video clips from a scene where each can contain from zero to multiple activities.
Normal instances are defined as background scene where normal human activities are there. Video clips that show humans with other objects like scooter or bicycle are defines are anomalies. 

Video clips are natural for MIL formulation as they are constructed from multiple frames. Here, length of clips identifies the bags length. We manually labelled video clips; so, the instance-level labels are not available for this dataset.
Our training and test sets contain 2000 images leads to 24 and 34 bags for train and test, respectively. We utilize the pre-trained InceptionV3 model on ImageNet ~\cite{szegedy2016rethinking} for feature extraction. By adding an extra layer of \emph{GlobalMaxPooling}, $2048$ features are obtained from each image.    

\subsubsection{Bridge Dataset}
This dataset contains both ambient and vehicle-induced vibration data collected from the Old ADA bridge in Japan. The bridge existed from 1959 to 2012. Before its removal, the vibration data was collected to serve as a real-world benchmark data for enhancing the research in structural health monitoring. Measurements are captured from five different states (ground-truth labels) of the bridge: 1) INT: no damage; 2) DMG1: half cut of one vertical member truss at the bridge midspan; 3) DMG2: fully cut of the same member; 4) RCV: recovered vertical member; 5) DMG3: fully cut of one vertical member at the bridge 5/8th span. The experiment was conducted at 200 Hz sampling rate and by means eight sensors ($A_{1}$ to $A_{8}$) in a way that three of them were installed on the opposite side of the damaged truss and five on the same side of it. Depending on a damage state, the test was repeated for various number of times. More details from the experiment can be found in~\cite{kim2021ambient}. Since ambient vibration is a preferable data due to its independence from any artificial loading, we consider this type of data in our analysis. Signals are segmented into $1$ second of measurements to generate the instances. It needs to be noted that RCV state is excluded from the experiment as its behavior needs further investigation.

We have included all three INT test repetitions in our analysis. First and third iterations are considered for training, but second one reserved for testing. $30$ seconds of measurements from normal and 60 seconds from damaged states are considered in our bag composition leading to 622 (21 training bags) and 1433 data points in train and test set (14 normal vs. 17 anomalous bags), respectively.

\subsection{Experimental Results}
In this section, we review the results of the MIL anomaly detection for all five datasets described above. To have a better understanding on how MIL helps, results are compared with StrOUD technique. The best AUC results obtained from each dataset for both StrOUD and MIL-StrOUD approaches are also reported. 

As mentioned earlier, There are some design decisions need to be determined for the framework. We choose LOF and autoencoder MSE as anomaly scores along with six aggregate functions described in \ref{sec:Methods} section. The corresponding hyperparameters for each setting are explained as follows. 

For both MIL-StrOUD and StrOUD, number of nearest neighbours needs to be specified when using LOF, but aggregate function is only needed for StrOUD due to its instance-level prediction. For all datasets same aggregate functions are employed, but number of neighbours depends on the number of instances in bags. So, this value is explained for each dataset separately.

In MSE setting, architecture of an autoencoder needs to be identified which is specified empirically for each dataset. 
Like in LOF, aggregate functions kept identical for all datasets here.


% Number of hidden layers, representation space, activation functions and batch sizes are among the hyperparameters need to be tuned for the framework when MSE is selected as an anomaly score. 


\subsubsection{CWRU}
As stated earlier, to provide a controlled setting for evaluating the robustness of the algorithm, various levels of Gaussian white noise are added to the signals. The lower a signal SNR, the higher the ratio of noise to a signal. 

Due to the existence of at least 10 instances in each bag, a range of $2$ to $10$ number of nearest neighbours is examined for LOF computation in MIL-StrOUD setting, but in StrOUD which there is no such a limitation, a larger range of values from $2$ to $50$ is considered.  

StrOUD and MIL-StrOUD results of CWRU for original and corrupted signals with both LOF and MSE scores are reported in table~\ref{CWRU-Results}.
The table indicates that no matter what anomaly score is selected,   both techniques are able to achieve the maximum AUC value (1.0) even in highly corrupted signals. This confirms that anomalies behave differently enough from normal data in CWRU dataset in such a way that they can be distinguished even if MIL has not been employed.

\begin{table}
\caption{Results of CWRU dataset for original and corrupted signals}
\label{CWRU-Results}
\begin{tabular}{ccccl}
\toprule
Method & Strangeness Factor & Signal & Best AUC\\
\midrule

MIL-StrOUD & LOF/MSE  & \begin{tabular}{@{}l@{}}
                   Original\\
                   SNR=20 db\\
                   SNR=10 db\\
                   SNR=5 db\\
                   SNR=1 db\\
                 \end{tabular} 

                & \begin{tabular}{@{}l@{}}
                   1.0\\
                   1.0\\
                   1.0\\
                   1.0\\
                   1.0\\
                 \end{tabular} \\
\hline
StrOUD & LOF/MSE  & \begin{tabular}{@{}l@{}}
                       Original\\
                       SNR=20 db\\
                       SNR=10 db\\
                       SNR=5 db\\
                       SNR=1 db\\
                     \end{tabular} 

                    & \begin{tabular}{@{}l@{}}
                       1.0\\
                       1.0\\
                       1.0\\
                       1.0\\
                       1.0\\
                     \end{tabular} \\

 \bottomrule
\end{tabular}
\end{table}



%--------
% \begin{table}
% \caption{MIL results of CWRU dataset for original and corrupted signals using LOF anomaly score}
% \label{CWRU-MIL-LOF}
% \begin{tabular}{ccccl}
% \toprule
% Signal & Number of nearest neighbours &  Aggregate function & Best AUC\\
% \midrule

% Original & 2 & dspread/maximum & 1.0\\
% SNR=20 db & 2  & dspread/maximum & 1.0 \\
% SNR=10 db & 2 & dspread/maximum & 1.0\\
% SNR=5 db & 2 & dspread/maximum & 1.0\\
% SNR=1 db & 2 & dspread/maximum & 1.0\\
%  \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}
% \caption{Non-MIL results of CWRU dataset for original and corrupted signals using LOF anomaly score}
% \label{CWRU-nonMIL-LOF}
% \begin{tabular}{cccl}
% \toprule
% Signal & Number of nearest neighbours  & Best AUC\\
% \midrule
% Original & 17 to 50  & 1.0\\
% SNR=20 db & 16 to 50  & 1.0 \\
% SNR=10 db & 2, 19 to 50  & 1.0\\
% SNR=5 db & 2, 19 to 50 & 1.0\\
% SNR=1 db & 2, 19 to 50 & 1.0\\
%  \bottomrule
% \end{tabular}
% \end{table}

% Results of MSE score are given in tables\ref{CWRU-MIL-MSE} and \ref{CWRU-MIL-MSE}. 

% \begin{table}
% \caption{MIL results of CWRU dataset for original and corrupted signals using MSE anomaly score}
% \label{CWRU-MIL-MSE}
% \begin{tabular}{cccl}
% \toprule
% Signal  &  Aggregate function & Best AUC\\
% \midrule

% Original  & spread & 1.0\\
% SNR=20 db & dspread& 1.0 \\
% SNR=10 db & dspread & 1.0\\
% SNR=5 db & dspread & 1.0\\
% SNR=1 db & dspread & 1.0\\
%  \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}
% \caption{Non-MIL results of CWRU dataset for original and corrupted signals using MSE anomaly score}
% \label{CWRU-MIL-MSE}
% \begin{tabular}{ccl}
% \toprule
% Signal & Best AUC\\
% \midrule

% Original & 1.0\\
% SNR=20 db & 1.0 \\
% SNR=10 db & 1.0\\
% SNR=5 db & 1.0\\
% SNR=1 db  & 1.0\\
%  \bottomrule
% \end{tabular}
% \end{table}

% The results show that regardless of added noise level or anomaly score, the maximum AUC value can be reached in CWRU. This confirms that anomalies behave differently enough from normal data in such a way that they can be distinguished no matter MIL has been utilized.      

\subsubsection{HAPT}
In HAPT dataset, we consider the similar range of neighbours for MIL setting (from $2$ to $10$), but a larger range of neighbours for StrOUD (from $2$ to $70$) as the dataset contains more data points compared to CWRU. Table~\cite{HAPT-Results} shows the results of both approaches.

As HAPT is a clean benchmark dataset, the results of both approaches are close. This means the extracted features are meaningful enough to distinguish postural transitions from other activities, and labels are accurately assigned to instances. Therefore, like CWRU, the StrOUD is enough for detecting anomalies in this dataset; although MIL can still produce slightly better results using either LOF or MSE score.  

\begin{table}
\caption{Results of HAPT dataset}
\label{HAPT-Results}
\begin{tabular}{ccccl}
\toprule
Method & Strangeness Factor & Best AUC\\
\midrule

MIL-StrOUD  & \begin{tabular}{@{}l@{}}
                   LOF\\
                   MSE\\
                 \end{tabular} 

            & \begin{tabular}{@{}l@{}}
                   0.996\\
                   0.994\\
                 \end{tabular} \\
\hline
StrOUD & \begin{tabular}{@{}l@{}}
           LOF\\
           MSE\\
         \end{tabular} 

        & \begin{tabular}{@{}l@{}}
           0.99\\
           0.98\\
         \end{tabular} \\

 \bottomrule
\end{tabular}
\end{table}
% \begin{table}
% \caption{MIL/Non-MIL results of HAPT dataset using LOF}\label{HAPT}
% \begin{tabular}{ccccl}
% \toprule
% MIL/Non-MIL & Number of nearest neighbours & Aggregate function & Best AUC\\
% \midrule
% MIL & 2 & maximum & 0.996 \\
% Non-MIL & 60 & -  & 0.99 \\
% \bottomrule
% \end{tabular}
% \end{table}

\subsubsection{Virat}
We assign bag labels manually based on the objects of the scene. However, instance-level labelling is ignored due to the complexity of the process. Results of the Virat dataset are given in table~\cite{Virat-Results}.

\begin{table}
\caption{Results of Virat dataset}
\label{Virat-Results}
\begin{tabular}{ccccl}
\toprule
Method & Strangeness Factor & Best AUC\\
\midrule

MIL-StrOUD  & \begin{tabular}{@{}l@{}}
                   LOF\\
                   MSE\\
                 \end{tabular} 

            & \begin{tabular}{@{}l@{}}
                   0.937\\
                   0.913\\
                 \end{tabular} \\

 \bottomrule
\end{tabular}
\end{table}

\subsubsection{Bridge}
According to the minimum number of instances in each bag ($30$), a range of $2$ to $20$ neighbours is examined for MIL experiment. This value is selected from $2$ to $50$ for StrOUD technique.

Table~\cite{bridge-Results} reports the results of ambient vibrations of Old ADA bridge dataset. It compares the results of MIL-StrOUD and StrOUD for all 8 sensors using LOF and MSE. It can be inferred from the table that using MIL approach enhances the results significantly. Low AUC values obtained from non-MIL experiments indicate that 
although the measurements are labeled according to the bridge health status, but they are not accurately assigned. The reason is that even though the bridge has been damaged, but most of the anomalous vibrations look like normal segments. The consequence is that data seems to be mislabelled. In other words, when we are dealing with raw real-world labeled datasets, evaluation becomes a challenging task due to the uncertainty about label accuracy. However, such an issue is alleviated by means of MIL technique which depends on group of instance labels. 

\begin{table}
\caption{Results of bridge dataset}
\label{bridge-Results}
\begin{tabular}{ccccl}
\toprule
Signal & Method & Strangeness Factor & Best AUC\\
\midrule
% ----- A1
%\begin{tabular}{@{}l@{}} 
%    \\ A1\\ \\ \\
%\end{tabular} & 

%\begin{tabular}{@{}l@{}}
%    \\ MIL-StrOUD\\ \\ StrOUD\\
%\end{tabular} & 

%\begin{tabular}{@{}l@{}}
%    LOF\\ MSE\\ LOF\\ MSE\\
%\end{tabular} & 

%\begin{tabular}{@{}l@{}} 
%    0.909\\ 0.850\\ 0.737\\ 0.769\\
%\end{tabular} \\

%\hline
% ----- A2
%\begin{tabular}{@{}l@{}}
%    \\ A2\\ \\ \\
%\end{tabular} & 

%\begin{tabular}{@{}l@{}}
%    \\ MIL-StrOUD\\ \\ StrOUD\\ 
%\end{tabular} &

%\begin{tabular}{@{}l@{}}
%    LOF\\ MSE\\ LOF\\ MSE\\
%\end{tabular} &

%\begin{tabular}{@{}l@{}}
%    0.877\\ 0.821\\ 0.678\\ 0.718
%\end{tabular} \\ 
%\hline
 %----- A3
%\begin{tabular}{@{}l@{}}
%    \\ A3\\ \\ \\
%\end{tabular} 
& 

\begin{tabular}{@{}l@{}}
    \\ MIL-StrOUD\\ \\ StrOUD\\ 
\end{tabular} &

\begin{tabular}{@{}l@{}}
    LOF\\ MSE\\ LOF\\ MSE\\
\end{tabular} &

\begin{tabular}{@{}l@{}}
    0.93\\ 0.905\\ 0.72\\ 0.739
\end{tabular} \\
\hline

% ----- A4
%\begin{tabular}{@{}l@{}}
%    \\ A4\\ \\ \\
%\end{tabular} & 

%\begin{tabular}{@{}l@{}}
%    \\ MIL-StrOUD\\ \\ StrOUD\\ 
%\end{tabular} &

%\begin{tabular}{@{}l@{}}
%    LOF\\ MSE\\ LOF\\ MSE\\
%\end{tabular} &

%\begin{tabular}{@{}l@{}}
%    0.861\\ 0.853\\ 0.631\\ 0.677
%\end{tabular} \\
%\hline
% ----- A5
%\begin{tabular}{@{}l@{}}
%    \\ A5\\ \\ \\
%\end{tabular} & 

%\begin{tabular}{@{}l@{}}
%    \\ MIL-StrOUD\\ \\ StrOUD\\ 
%\end{tabular} &

%\begin{tabular}{@{}l@{}}
%    LOF\\ MSE\\ LOF\\ MSE\\
%\end{tabular} &

%\begin{tabular}{@{}l@{}}
%    0.7\\ 0.756\\ 0.552\\ 0.574
%\end{tabular} \\
%\hline
% ----- A6
%\begin{tabular}{@{}l@{}}
%    \\ A6\\ \\ \\
%\end{tabular} & 

%\begin{tabular}{@{}l@{}}
%    \\ MIL-StrOUD\\ \\ StrOUD\\ 
%\end{tabular} &

%\begin{tabular}{@{}l@{}}
%    LOF\\ MSE\\ LOF\\ MSE\\
%\end{tabular} &

%\begin{tabular}{@{}l@{}}
%    0.992\\ 0.976\\ 0.898\\ 0.904
%\end{tabular} \\
%\hline
% ----- A7
%\begin{tabular}{@{}l@{}}
%    \\ A7 \\ \\ \\
%\end{tabular} & 

%\begin{tabular}{@{}l@{}}
%    \\ MIL-StrOUD\\ \\ StrOUD\\ 
%\end{tabular} &

%\begin{tabular}{@{}l@{}}
%    LOF\\ MSE\\ LOF\\ MSE\\
%\end{tabular} &

%\begin{tabular}{@{}l@{}}
%    0.962\\ 0.988\\ 0.908\\ 0.915
%\end{tabular} \\
%\hline
% ----- A8
%\begin{tabular}{@{}l@{}}
%    \\ A8 \\ \\ \\
%\end{tabular} & 

%\begin{tabular}{@{}l@{}}
%    \\ MIL-StrOUD\\ \\ StrOUD\\ 
%\end{tabular} &

%\begin{tabular}{@{}l@{}}
%    LOF\\ MSE\\ LOF\\ MSE\\
%\end{tabular} &

%\begin{tabular}{@{}l@{}}
%    0.923\\ 0.98\\ 0.875\\ 0.9
%\end{tabular} \\
\bottomrule
\end{tabular}
\end{table}






% \begin{table}
% \caption{MIL results of bridge dataset using LOF}\label{bridge-MIL-LOF}
% \begin{tabular}{ccccl}
% \toprule
% Sensor & Number of nearest neighbours & Aggregate function & Best AUC\\
% \midrule
% A1 & 8 & maximum & 0.909 \\
% A2 & 2 & maximum & 0.877 \\
% A3 & 2 & maximum & 0.93 \\
% A4 & 12 & maximum & 0.861 \\ 
% A5 & 4 & maximum & 0.7 \\
% A6 & 13 & spread & 0.992 \\
% A7 & 19 & maximum & 0.962 \\
% A8 & 15 & ave & 0.923 \\

% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}
% \caption{Non-MIL results of bridge dataset using LOF}\label{bridge-nonMIL-LOF}
% \begin{tabular}{cccl}
% \toprule
% Sensor & Number of nearest neighbours & Best AUC\\
% \midrule
% A1 & 5  & 0.737 \\
% A2 & 4  & 0.678 \\
% A3 & 10  & 0.72 \\
% A4 & 15  & 0.631 \\ 
% A5 & 3  & 0.552 \\
% A6 & 14  & 0.898 \\
% A7 & 50  & 0.908 \\
% A8 & 22  & 0.875 \\

% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}
% \caption{MIL results of bridge dataset using MSE}\label{bridge-MIL-MSE}
% \begin{tabular}{cccl}
% \toprule
% Sensor Number & Aggregate function & Best AUC\\
% \midrule
% A1 & median & 0.850 \\
% A2 & maximum & 0.821 \\
% A3 & maximum & 0.905 \\
% A4 & maximum & 0.853 \\ 
% A5 & maximum & 0.756 \\
% A6 & dspread & 0.976 \\
% A7 & spread & 0.988 \\
% A8 & ave & 0.98 \\

% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}
% \caption{Non-MIL results of bridge dataset using MSE}\label{bridge-nonMIL-MSE}
% \begin{tabular}{ccl}
% \toprule
% Sensor Number & Best AUC\\
% \midrule
% A1 & 0.769 \\
% A2 & 0.718 \\
% A3 & 0.739 \\
% A4 & 0.677 \\ 
% A5 & 0.574 \\
% A6 & 0.904 \\
% A7 & 0.915 \\
% A8 & 0.900 \\

% \bottomrule
% \end{tabular}
% \end{table}


